Stellar population astrophysics (SPA) with the TNG -- The chemical content of the red supergiant population in the Perseus complex

Context. The Perseus complex in the outer disk of the Galaxy hosts a number of clusters and associations of young stars. Gaia is providing a detailed characterization of their kinematic structure and evolutionary properties. Aims. Within the SPA Large Programme at the TNG, we secured HARPS-N and GIANO-B high-resolution optical and near-infrared (NIR) spectra of the young red supergiant (RSG) stars in the Perseus complex, in order to obtain accurate radial velocities, stellar parameters and detailed chemical abundances. Methods. We used spectral synthesis to best-fit hundreds of atomic and molecular lines in the spectra of the observed 27 RSGs. We obtained accurate estimates of the stellar temperature, gravity, micro and macro turbulence velocities and chemical abundances for 25 different elements. We also measured the $^{12}$C/$^{13}$C abundance ratio. Results. Our combined optical and NIR chemical study provides homogeneous half-solar iron with a small dispersion, about solar-scaled abundance ratios for the iron-peak, alpha and other light elements and a small enhancement of Na, K and neutron-capture elements, consistent with the thin disk chemistry traced by older stellar populations at a similar Galactocentric distance of about 10 kpc. We inferred enhancement of N, depletion of C and of the $^{12}$C/$^{13}$C isotopic abundance ratio, consistent with mixing processes in the stellar interiors during the RSG evolution.

==> Perseus Complex (ArXiv)/tab1.tex <==
\begin{table*}[h]
\centering
\tiny
\addtolength{\tabcolsep}{-1.7pt}    
\caption{Photometric information for the studied RSGs and derived stellar parameters and RVs.}
\label{tab_obs} 
\begin{tabular}{|l|l|cc|rrr|c|c|c||ccc|c|}
\hline
 \# & star & RA(J2000) & DEC(J2000) & \multicolumn{3}{c|}{Gaia EDR3} & 2MASS & E(B-V) & $\rm log\Big(\frac{L_{Bol}}{L_{\odot}}\Big)$  &  $T_{eff}$ & log(g)  & $\xi$ &  RV\\
 & & (h : m : s) &  ($^o$ : ' : '') & G & BP & RP & K & & & [K]  &  [dex]   &  [$\rm km \ s^{-1}$]   & [$\rm km \ s^{-1}$] \\
\hline
\rowcolor{lightgray}
1 & SU Per  & 2:22:06.9 & 56:36:14.9  & 5.93 & 7.70 & 4.70 & 1.46 & 0.36 & 4.95 & 3466 & -0.37 & 3.80 & -49\\
2 & FZ Per & 2:20:59.6 & 57:09:29.9  & 6.86 & 8.30 & 5.67 & 2.48 & 0.51 & 4.64 & 3750 &  0.07 & 3.10 & -44 \\
\rowcolor{lightgray}
3 & V439 Per & 2:23:11.1 & 57:11:57.9  & 7.00 & 8.43 & 5.86 & 2.69 & 0.55 & 4.44 & 3690 &  0.25 & 3.40 & -44  \\
4 & V550 Per & 2:15:13.3 & 58:08:32.4  & 7.59 & 9.10 & 6.41 & 3.19 & 0.74 & 4.62 & 3720 &  0.08 & 3.30 & -47 \\
\rowcolor{lightgray}
5 & PP Per & 2:17:08.2 & 58:31:47.0  & 7.74 & 9.48 & 6.52 & 2.95 & 0.78 & 4.50 & 3670 &  0.18 & 3.00 & -51 \\
6 & BD+57 540 & 2:19:46.9 & 58:38:48.1  & 8.28 & 9.51 & 7.19 & 4.28 & 0.68 & 4.18 & 4125 &  0.70 & 2.10 & -53 \\
\rowcolor{lightgray}
7 & HD 15406 & 2:30:45.7 & 55:56:53.2  & 8.68 & 9.69 & 7.71 & 5.15 & 0.40 & 3.96 & 4190 &  0.95 & 2.00 & -51 \\
8  & YZ Per   & 2:38:25.4 & 57:02:46.2 & 6.45 & 8.17 & 5.28 & 1.91 & 0.62 & 4.85 & 3616 & -0.20 & 4.00 & -43 \\
\rowcolor{lightgray} 
9 & T Per    & 2:19:21.9 & 58:57:40.4 & 7.19 & 8.88 & 5.91 & 1.94 & 0.84 & 4.63 & 3594 &  0.01 & 3.30 & -41 \\
10  & GP Cas & 2:39:50.4 & 59:35:51.3 & 7.45 & 9.76 & 6.10 & 1.95 & 1.07 & 4.74 & 3471 & -0.16 & 3.40 & -41 \\
\rowcolor{lightgray} 
11  & BD+60 299 & 1:39:51.7 & 60:54:08.3 & 6.44 & 8.05 & 5.18 & 2.11 & 0.75 & 5.05 & 3491 & -0.45 & 3.40 & -44 \\
12  & V648 Cas & 2:51:03.9 & 57:51:19.9 & 7.52 & 9.70 & 6.08 & 2.25 & 1.27 & 4.87 & 3572 & -0.24 & 3.50 & -41 \\
\rowcolor{lightgray} 
13 & DO 26429 & 0:56:53.2 & 57:33:24.9 & 7.86 & 10.09 & 6.49 & 2.48 & 1.49 & 4.94 & 3578 & -0.30 & 3.50 & -42 \\
14 & V605 Cas & 2:20:22.5 & 59:40:16.9 & 7.02 & 8.73 & 5.87 & 2.58 & 0.82 & 4.95 & 3736 & -0.24 & 3.10 & -36 \\
\rowcolor{lightgray} 
15  & BD+60 265 & 1:33:33.2 & 61:33:29.7 & 7.23 & 8.79 & 6.05 & 2.63 & 0.88 & 4.61 & 3637 &  0.06 & 3.20 & -41 \\
16  & BD+60 327 & 1:45:38.8 & 61:02:22.8 & 7.08 & 8.49 & 5.93 & 2.93 & 1.26 & 4.58 & 3778 &  0.15 & 3.00 & -46 \\
\rowcolor{lightgray} 
17 & HD 237006 & 2:49:08.8 & 58:00:48.4 & 7.86 & 9.35 & 6.66 & 3.12 & 1.10 & 4.40 & 3863 &  0.37 & 2.80 & -39 \\
18 & BD+59274 & 1:33:29.2 & 60:38:47.7 & 7.44 & 8.79 & 6.31 & 3.12 & 0.51 & 4.62 & 3740 &  0.09 & 2.80 & -45 \\
\rowcolor{lightgray} 
19  & WX Cas   & 1:54:03.7 & 61:06:32.9 & 8.46 & 10.20 & 7.24 & 3.41 & 1.88 & 4.50 & 3787 &  0.23 & 3.00 & -44 \\
20 & IRAS02414+5752 & 2:45:12.2 & 58:05:24.4 & 8.27 & 9.91 & 7.07 & 3.56 & 0.89 & 4.42 & 3850 &  0.34 & 2.60 & -42 \\
\rowcolor{lightgray} 
21  & IRAS01530+6149 & 1:56:35.8 & 62:04:13.2 & 8.19 & 9.81 & 6.97 & 3.74 & 1.04 & 4.49 & 3793 &  0.25 & 2.60 & -45 \\
22  & BD+61 369 & 2:03:08.2 & 62:11:24.0 & 7.85 & 9.25 & 6.72 & 3.78 & 1.06 & 4.24 & 3869 &  0.53 & 2.60 & -44 \\
\rowcolor{lightgray} 
23  & DO 24697 & 1:44:38.3 & 61:37:43.2 & 8.58 & 10.21 & 7.37 & 3.87 & 1.62 & 4.29 & 3896 &  0.50 & 2.40 & -37 \\
24  & BD+60 287 & 1:38:03.6 & 61:02:49.2 & 7.90 & 9.16 & 6.81 & 3.98 & 0.73 & 4.04 & 4009 &  0.79 & 2.50 & -44 \\
\rowcolor{lightgray} 
25  & BD+62 272 & 1:34:52.3 & 62:46:28.8 & 8.42 & 9.73 & 7.31 & 4.20 & 1.18 & 4.34 & 3925 &  0.46 & 2.40 & -40 \\
26  & BD+59 532 & 2:42:56.9 & 60:12:16.1 & 8.80 & 10.35 & 7.62 & 4.20 & 1.08 & 4.14 & 4016 &  0.69 & 2.40 & -44 \\
\rowcolor{lightgray} 
27  & IRAS02476+5850 & 2:51:27.1 & 59:02:34.3 & 9.47 & 10.75 & 8.37 & 5.28 & 0.99 & 3.94 & 4048 &  0.91 & 2.30 & -31 \\
\hline\hline
\end{tabular}
\end{table*}



==> Perseus Complex (ArXiv)/tab2.tex <==
\begin{landscape}
\begin{table}[t]
\centering
\caption{CNO, F, Na, Al, K and alpha element abundances for the studied RSGs in the Perseus complex. Values are solar-scaled according to \citet{Grevesse98} solar reference, with the only exception of oxygen for which we used \citet{Asplund09}. Numbers in parenthesis represent the number of lines used to determine chemical abundances.}
\scriptsize
\addtolength{\tabcolsep}{-4.5pt}    
\begin{tabular}{|l|c|c|c|cc|c|cc|cc|c||cc|cc|c|cc|cc|c|cc|}
\hline
\# & [C/H] & $^{12}$C/$^{13}$C& [N/H] & \multicolumn{2}{c|}{[O/H]}& [F/H]& \multicolumn{2}{c|}{[Na/H]}& \multicolumn{2}{c|}{[Al/H]} &[K/H] & \multicolumn{2}{c|}{[Mg/H]}& \multicolumn{2}{c|}{[Si/H]}& [S/H] & \multicolumn{2}{c|}{[Ca/H]} & \multicolumn{2}{c|}{[ScI/H]} & [ScII/H] & \multicolumn{2}{c|}{[Ti/H]} \\ 
& NIR & NIR & NIR & NIR & OPT & NIR & NIR & OPT & NIR & OPT & NIR &NIR & OPT& NIR & OPT & NIR & NIR & OPT & NIR & OPT & OPT & NIR & OPT \\
\hline
\rowcolor{lightgray}			
1      & -0.54 (29)  &  7.00 ( 2)  &  0.26 (18)  & -0.33 (17)  &     --      & -0.50 ( 1)  & -0.15 ( 3)  &      --     & -0.33 ( 4)  &      --     & -0.14 ( 1)    & -0.29 ( 4)  & -0.38 ( 2)  & -0.31 (11)  &      --     & -0.14 ( 1)  & -0.32 (10)  &      --     & -0.32 ( 3)   &      --     &      --      & -0.40 (11)  &      --	\\ 
\rowcolor{lightgray} 																 
   &  $\pm$ 0.05 &  $\pm$ 1.50 &  $\pm$ 0.04 &  $\pm$ 0.02 &     --          &  $\pm$ 0.10 &  $\pm$ 0.07 &      --     &  $\pm$ 0.08 &      --     &  $\pm$ 0.10   &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.04 &      --     &  $\pm$ 0.10 &  $\pm$ 0.06 &      --     &  $\pm$ 0.09  &      --     &      --      &  $\pm$ 0.05 &      --	\\ 
2     & -0.58 (45)  &  8.00 ( 2)  &  0.05 (54)  & -0.35 (34)  &     --       & -0.58 ( 1)  & -0.20 ( 3)  & -0.25 ( 2)  & -0.41 ( 4)  & -0.36 ( 2)  & -0.28 ( 1)    & -0.37 ( 3)  & -0.38 ( 2)  & -0.29 (12)  & -0.39 ( 2)  & -0.36 ( 5)  & -0.31 (14)  & -0.29 ( 3)  & -0.32 ( 5)   & -0.43 ( 4)  &      --      & -0.47 (16)  & -0.35 (17)   \\  
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.02 &  $\pm$ 0.01 &     --          &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.05 &  $\pm$ 0.07 &  $\pm$ 0.08  &  $\pm$ 0.02 &      --      &  $\pm$ 0.04 &  $\pm$ 0.01	\\ 
\rowcolor{lightgray} 																 
3     & -0.55 (43)  &  8.00 ( 2)  &  0.10 (61)  & -0.37 (31)  &     --       & -0.56 ( 1)  & -0.14 ( 3)  & -0.20 ( 2)  & -0.35 ( 4)  & -0.32 ( 2)  & -0.31 ( 1)    & -0.27 ( 4)  & -0.25 ( 2)  & -0.25 (10)  & -0.25 ( 2)  & -0.37 ( 2)  & -0.28 (13)  & -0.29 ( 5)  & -0.34 ( 4)   & -0.43 ( 3)  &      --      & -0.47 (16)  & -0.35 (17)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.02 &  $\pm$ 0.01 &     --          &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.07 &  $\pm$ 0.09  &  $\pm$ 0.02 &      --      &  $\pm$ 0.04 &  $\pm$ 0.01	\\ 
4     & -0.66 (37)  & 11.00 ( 2)  &  0.10 (58)  & -0.34 (16)  &     --       & -0.63 ( 1)  & -0.26 ( 3)  & -0.18 ( 2)  & -0.50 ( 5)  & -0.33 ( 2)  & -0.33 ( 1)    & -0.40 ( 4)  & -0.36 ( 2)  & -0.28 (12)  & -0.33 ( 2)  & -0.31 ( 2)  & -0.28 (12)  & -0.35 ( 5)  & -0.43 ( 6)   &      --     &      --      & -0.44 (15) & -0.42 (25)   \\  
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.01 &  $\pm$ 0.01 &     --          &  $\pm$ 0.10 &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.04 &  $\pm$ 0.08  &      --     &      --      &  $\pm$ 0.04 &  $\pm$ 0.02	\\ 
\rowcolor{lightgray} 																 
5     & -0.56 (39)  & 10.00 ( 2)  &  0.10 (56)  & -0.34 (13)  &     --       & -0.53 ( 1)  & -0.10 ( 3)  & -0.05 ( 2)  & -0.24 ( 5)  & -0.37 ( 2)  & -0.17 ( 1)    & -0.27 ( 4)  & -0.26 ( 2)  & -0.22 (11)  & -0.25 ( 2)  & -0.33 ( 3)  & -0.25 (12)  & -0.36 ( 5)  & -0.33 ( 3)   & -0.38 ( 4)  &      --      & -0.44 (16)  & -0.36 (22)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.01 &  $\pm$ 0.01 &     --          &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.03 &  $\pm$ 0.04 &  $\pm$ 0.15  &  $\pm$ 0.04 &      --      &  $\pm$ 0.04 &  $\pm$ 0.02	\\ 
6     & -0.34 (36)  & 29.00 ( 2)  & -0.28 (62)  & -0.23 (13)  & -0.24 ( 1)   & -0.39 ( 1)  & -0.31 ( 3)  & -0.29 ( 2)  & -0.22 ( 5)  & -0.20 ( 2)  & -0.09 ( 1)    & -0.28 ( 7)  & -0.32 ( 2)  & -0.23 (25)  & -0.29 ( 2)  & -0.35 ( 7)  & -0.26 ( 9)  & -0.33 ( 5)  & -0.32 ( 5)   & -0.25 ( 4)  &      --      & -0.32 (28)  & -0.29 (22)   \\  
   &  $\pm$ 0.01 &  $\pm$ 1.50 &  $\pm$ 0.01 &  $\pm$ 0.01 &  $\pm$ 0.10     &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.04 &  $\pm$ 0.09 &  $\pm$ 0.10  &  $\pm$ 0.07 &      --      &  $\pm$ 0.03 &  $\pm$ 0.03	\\ 
\rowcolor{lightgray} 																 
7     & -0.38 (28)  & 23.00 ( 2)  & -0.18 (56)  & -0.16 (16)  & -0.20 ( 1)   & -0.43 ( 1)  &  0.07 ( 3)  & -0.01 ( 2)  & -0.23 ( 2)  & -0.20 ( 2)  &  0.00 ( 1)    & -0.17 ( 9)  & -0.32 ( 2)  & -0.15 (30)  & -0.29 ( 2)  & -0.34 ( 7)  & -0.16 ( 9)  & -0.33 ( 5)  & -0.26 ( 3)   & -0.25 ( 4)  &      --      & -0.23 (27)  & -0.29 (22)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.02 &  $\pm$ 1.50 &  $\pm$ 0.01 &  $\pm$ 0.01 &  $\pm$ 0.10     &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.03 &  $\pm$ 0.11 &  $\pm$ 0.03  &  $\pm$ 0.04 &      --      &  $\pm$ 0.02 &  $\pm$ 0.01	\\ 
8     & -0.55 (31)  &  7.00 ( 2)  & -0.12 (56)  & -0.30 (21)  &     --       & -0.59 ( 1)  & -0.23 ( 3)  & -0.26 ( 3)  & -0.31 ( 3)  & -0.34 ( 3)  & -0.25 ( 1)    & -0.31 ( 3)  & -0.30 ( 2)  & -0.23 (12)  & -0.31 ( 2)  & -0.41 ( 1)  & -0.30 (13)  & -0.40 ( 5)  & -0.41 ( 5)   & -0.47 ( 4)  & -0.37 ( 8)   & -0.43 (28)  & -0.45 (19)   \\  
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.01 &  $\pm$ 0.01 &     --          &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.10   &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.07 &  $\pm$ 0.04  &  $\pm$ 0.03 &  $\pm$ 0.03  &  $\pm$ 0.03 &  $\pm$ 0.02	\\ 
\rowcolor{lightgray} 																 
9    & -0.51 (35)  &  7.00 ( 2)  & -0.08 (58)  & -0.33 (21)  &     --        & -0.59 ( 1)  & -0.29 ( 3)  & -0.33 ( 3)  & -0.28 ( 3)  & -0.34 ( 2)  & -0.23 ( 1)    & -0.28 ( 3)  & -0.30 ( 2)  & -0.21 (11)  & -0.22 ( 1)  & -0.31 ( 2)  & -0.32 (11)  & -0.31 ( 5)  & -0.31 ( 5)   & -0.44 ( 3)  & -0.43 ( 8)   & -0.46 (27)  & -0.45 (17)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.01 &  $\pm$ 1.50 &  $\pm$ 0.01   &  $\pm$ 0.01 &     --        &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.08 &  $\pm$ 0.06 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.07 &  $\pm$ 0.06  &  $\pm$ 0.03 &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.05	\\ 
10    & -0.45 (33)  &  9.00 ( 2)  & -0.03 (51) & -0.18 (19)  &     --        & -0.35 ( 1)  & -0.07 ( 3)  & -0.04 ( 2)  & -0.21 ( 1)  & -0.17 ( 3)  & -0.08 ( 1)    & -0.24 ( 3)  & -0.24 ( 2)  & -0.18 (11)  & -0.25 ( 2)  & -0.33 ( 3)  & -0.21 ( 9)  & -0.24 ( 4)  & -0.23 ( 3)   & -0.39 ( 3)  & -0.37 ( 8)   & -0.25 (25)  & -0.31 (19)   \\  
   &  $\pm$ 0.01 &  $\pm$ 1.50 &  $\pm$ 0.01   &  $\pm$ 0.01 &     --        &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.16 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.10   &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.04 &  $\pm$ 0.09 &  $\pm$ 0.03  &  $\pm$ 0.04 &  $\pm$ 0.03  &  $\pm$ 0.02 &  $\pm$ 0.02	\\ 
\rowcolor{lightgray} 																 
11    & -0.49 (31)  &  6.00 ( 2)  & -0.06 (57) & -0.13 (21)  &     --        & -0.25 ( 1)  & -0.10 ( 3)  & -0.20 ( 1)  & -0.22 ( 2)  & -0.22 ( 3)  & -0.09 ( 1)    & -0.27 ( 3)  & -0.30 ( 2)  & -0.31 (12)  & -0.31 ( 1)  & -0.30 ( 3)  & -0.30 (11)  & -0.39 ( 4)  & -0.15 ( 3)   & -0.32 ( 2)  & -0.46 ( 6)   & -0.20 (25)  & -0.26 (16)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.01 &  $\pm$ 1.50 &  $\pm$ 0.01   &  $\pm$ 0.01 &     --        &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.10   &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.03 &  $\pm$ 0.09 &  $\pm$ 0.05  &  $\pm$ 0.10 &  $\pm$ 0.08  &  $\pm$ 0.03 &  $\pm$ 0.03	\\ 
12   & -0.48 (28)  &  9.00 ( 2)  &  0.02 (54)  & -0.20 (21)  &     --        & -0.38 ( 1)  & -0.04 ( 3)  & -0.13 ( 2)  & -0.21 ( 3)  & -0.23 ( 3)  & -0.12 ( 1)    & -0.28 ( 3)  & -0.30 ( 2)  & -0.29 (12)  & -0.35 ( 2)  & -0.18 ( 3)  & -0.27 (11)  & -0.34 ( 5)  & -0.27 ( 3)   & -0.35 ( 4)  & -0.36 ( 8)   & -0.33 (25)  & -0.31 (20)   \\  
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.02   &  $\pm$ 0.01 &     --        &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.08 &  $\pm$ 0.06 &  $\pm$ 0.06 &  $\pm$ 0.10    &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.02 &  $\pm$ 0.09 &  $\pm$ 0.04  &  $\pm$ 0.04 &  $\pm$ 0.03  &  $\pm$ 0.02 &  $\pm$ 0.02	\\ 
\rowcolor{lightgray} 																 
13   & -0.50 (28)  &  8.00 ( 2)  &  0.02 (55)  & -0.25 (20)  &     --        & -0.31 ( 1)  & -0.02 ( 3)  & -0.04 ( 1)  & -0.33 ( 1)  & -0.27 ( 2)  & -0.15 ( 1)    & -0.28 ( 3)  & -0.30 ( 2)  & -0.25 (10)  & -0.27 ( 2)  & -0.25 ( 3)  & -0.24 (11)  & -0.28 ( 5)  & -0.27 ( 4)   & -0.42 ( 4)  & -0.45 ( 8)   & -0.36 (23)  & -0.38 (22)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.02   &  $\pm$ 0.01 &     --        &  $\pm$ 0.10 &  $\pm$ 0.01 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.03 &  $\pm$ 0.05 &  $\pm$ 0.03  &  $\pm$ 0.03 &  $\pm$ 0.03  &  $\pm$ 0.02 &  $\pm$ 0.02	\\ 
14   & -0.49 (38)  &  9.00 ( 2)  &  0.01 (55)  & -0.24 (21)  &     --        & -0.42 ( 1)  & -0.22 ( 3)  & -0.29 ( 2)  & -0.33 ( 3)  & -0.36 ( 2)  & -0.17 ( 1)    & -0.32 ( 3)  & -0.30 ( 2)  & -0.25 (14)  & -0.28 ( 1)  & -0.24 ( 5)  & -0.27 (12)  & -0.34 ( 2)  & -0.32 ( 3)   & -0.41 ( 4)  & -0.52 ( 5)   & -0.35 (32)  & -0.39 (17)   \\  
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.02   &  $\pm$ 0.01 &     --        &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.05  &  $\pm$ 0.01 &  $\pm$ 0.08  &  $\pm$ 0.02 &  $\pm$ 0.05	\\ 
\rowcolor{lightgray} 																 
15    & -0.42 (27)  & 16.00 ( 2)  & -0.09 (57)  & -0.13 (17)  &     --       & -0.21 ( 1)  &  0.01 ( 3)  & -0.05 ( 2)  & -0.15 ( 1)  & -0.23 ( 3)  & -0.08 ( 1)    & -0.29 ( 3)  & -0.28 ( 2)  & -0.28 (12)  & -0.27 ( 2)  & -0.21 ( 3)  & -0.25 (10)  & -0.30 ( 5)  & -0.17 ( 3)   & -0.29 ( 3)  & -0.32 ( 8)   & -0.22 (23)  & -0.32 (15)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.02    &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.10   &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.03 &  $\pm$ 0.08 &  $\pm$ 0.03  &  $\pm$ 0.08 &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.03	\\ 
16    & -0.55 (27)  & 22.00 ( 2)  &  0.30 (26)  & -0.38 (21)  &     --       & -0.88 ( 1)  & -0.02 ( 3)  &     --      & -0.35 ( 3)  &     --      & -0.21 ( 1)    & -0.23 ( 3)  & -0.29 ( 2)  & -0.08 (13)  &     --      & -0.19 ( 2)  & -0.26 (12)  &     --      & -0.38 ( 4)   &     --      &      --      & -0.53 (29)  &     --      \\  
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.03    &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.09 &     --      &  $\pm$ 0.08 &     --      &  $\pm$ 0.10   &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.06 &     --      &  $\pm$ 0.10 &  $\pm$ 0.04 &     --      &  $\pm$ 0.09  &     --      &      --      &  $\pm$ 0.02 &     --	\\ 
\rowcolor{lightgray} 																 
17   & -0.52 (34)  & 17.00 ( 2)  &  0.10 (38)   & -0.36 (21)  &     --       & -0.77 ( 1)  & -0.14 ( 3)  & -0.15 ( 1)  & -0.38 ( 3)  & -0.39 ( 2)  & -0.32 ( 1)    & -0.32 ( 3)  & -0.29 ( 2)  & -0.21 (12)  & -0.29 ( 2)  & -0.09 ( 3)  & -0.36 (13)  & -0.35 ( 5)  & -0.37 ( 5)   & -0.47 ( 2)  & -0.41 ( 5)   & -0.45 (28)  & -0.46 (18)   \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.02 &  $\pm$ 0.01    &     --       &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.06  &  $\pm$ 0.10 &  $\pm$ 0.04  &  $\pm$ 0.01 &  $\pm$ 0.01	\\ 
18    & -0.45 (33)  & 10.00 ( 2)  &  0.02 (58)  & -0.23 (19)  &     --       & -0.53 ( 1)  & -0.18 ( 2)  & -0.21 ( 3)  & -0.16 ( 3)  & -0.19 ( 3)  & -0.16 ( 1)    & -0.26 ( 3)  & -0.16 ( 2)  & -0.19 (13)  & -0.13 ( 2)  & -0.26 ( 5)  & -0.27 (12)  & -0.30 ( 4)  & -0.35 ( 5)   & -0.34 ( 4)  & -0.21 ( 8)   & -0.38 (29)  & -0.38 (21)   \\  
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.01 &  $\pm$ 0.01    &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.04 &  $\pm$ 0.05 &  $\pm$ 0.10   &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.04 &  $\pm$ 0.05 &  $\pm$ 0.03  &  $\pm$ 0.03 &  $\pm$ 0.10  &  $\pm$ 0.02 &  $\pm$ 0.01	\\ 
\rowcolor{lightgray} 																 
19    & -0.53 (30)  & 12.00 ( 2)  &  0.28 (43)  & -0.43 (20)  &     --       & -0.81 ( 1)  &  0.02 ( 1)  &     --      & -0.49 ( 3)  &     --      & -0.45 ( 1)    & -0.38 ( 2)  & -0.31 ( 1)  & -0.24 ( 9)  &     --      & -0.25 ( 3)  & -0.41 ( 7)  &     --      & -0.29 ( 4)   &     --      &      --      & -0.52 (19)  &     --      \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.03    &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &     --      &  $\pm$ 0.08 &     --      &  $\pm$ 0.10   &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.04 &     --      &  $\pm$ 0.04 &  $\pm$ 0.03 &     --      &  $\pm$ 0.05  &     --      &      --      &  $\pm$ 0.02 &     --	\\ 
20   & -0.47 (26)  &  9.00 ( 2)  &  0.03 (51)   & -0.22 (21)  & -0.18 ( 1)   & -0.42 ( 1)  &  0.08 ( 1)  &  0.04 ( 2)  & -0.15 ( 2)  & -0.22 ( 3)  & -0.09 ( 1)    & -0.29 ( 3)  & -0.31 ( 2)  & -0.28 (10)  & -0.33 ( 2)  & -0.24 ( 3)  & -0.28 ( 9)  & -0.32 ( 4)  & -0.22 ( 3)   & -0.26 ( 4)  & -0.30 ( 7)   & -0.25 (26)  & -0.28 (14)   \\  
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.01    & $\pm$ 0.01  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.10   &  $\pm$ 0.06 &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.02 &  $\pm$ 0.08 &  $\pm$ 0.04  &  $\pm$ 0.04 &  $\pm$ 0.10  &  $\pm$ 0.02 &  $\pm$ 0.04	\\ 
\rowcolor{lightgray} 																
21    & -0.43 (27)  & 13.00 ( 2)  &  0.28 (28)  & -0.26 (21)  &     --       & -0.56 ( 1)  & -0.04 ( 1)  &     --      & -0.09 ( 2)  &     --      & -0.24 ( 1)    & -0.28 ( 3)  & -0.36 ( 2)  & -0.21 (13)  &     --      & -0.27 ( 2)  & -0.32 (10)  &     --      & -0.35 ( 2)   &     --      &      --      & -0.46 (30)  &     --      \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.03    &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &     --      &  $\pm$ 0.10 &     --      &  $\pm$ 0.10   &  $\pm$ 0.08 &  $\pm$ 0.10 &  $\pm$ 0.08 &     --      &  $\pm$ 0.10 &  $\pm$ 0.04 &     --      &  $\pm$ 0.10  &     --      &      --      &  $\pm$ 0.02 &     --	\\ 
22    & -0.46 (28)  & 17.00 ( 2)  & -0.01 (56)  & -0.13 (16)  &     --       & -0.24 ( 1)  &  0.00 ( 1)  & -0.18 ( 1)  & -0.25 ( 2)  & -0.37 ( 2)  & -0.20 ( 1)    & -0.31 ( 3)  & -0.31 ( 2)  & -0.31 (10)  & -0.35 ( 2)  & -0.34 ( 3)  & -0.28 (12)  & -0.35 ( 3)  & -0.26 ( 1)   & -0.33 ( 3)  & -0.33 ( 4)   & -0.28 (26)  & -0.43 (10)   \\  
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.01    &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.06 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.02 &  $\pm$ 0.08  &  $\pm$ 0.02 &  $\pm$ 0.02	\\ 
\rowcolor{lightgray} 																 
23    & -0.47 (37)  & 19.00 ( 2)  &  0.25 (26)  & -0.37 (21)  &     --       & -0.46 ( 1)  & -0.04 ( 1)  &     --      & -0.15 ( 3)  &     --      & -0.27 ( 1)    & -0.27 ( 3)  & -0.30 ( 1)  & -0.22 (12)  &     --      & -0.19 ( 2)  & -0.26 (11)  &     --      & -0.34 ( 2)   &     --      &      --      & -0.44 (28)  &     --      \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.01 &  $\pm$ 1.00 &  $\pm$ 0.02    &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &     --      &  $\pm$ 0.01 &     --      &  $\pm$ 0.10   &  $\pm$ 0.07 &  $\pm$ 0.10 &  $\pm$ 0.04 &     --      &  $\pm$ 0.10 &  $\pm$ 0.04 &     --      &  $\pm$ 0.10  &     --      &      --      &  $\pm$ 0.02 &     --	\\ 
24    & -0.43 (23)  & 21.00 ( 2)  & -0.05 (57)  & -0.19 (19)  &     --       & -0.41 ( 1)  & -0.18 ( 1)  & -0.16 ( 3)  & -0.10 ( 4)  & -0.19 ( 3)  & -0.14 ( 1)    & -0.30 ( 2)  & -0.27 ( 2)  & -0.19 (12)  & -0.23 ( 2)  & -0.24 ( 2)  & -0.28 (11)  & -0.32 ( 5)  & -0.26 ( 5)   & -0.34 ( 4)  & -0.27 ( 7)   & -0.34 (27)  & -0.37 (22)   \\  
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.01    &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.01 &  $\pm$ 0.06 &  $\pm$ 0.10   &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.08 &  $\pm$ 0.07  &  $\pm$ 0.03 &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.02	\\ 
\rowcolor{lightgray} 																 
25    & -0.50 (20)  & 14.00 ( 2)  &  0.29 (15)  & -0.27 (18)  &     --       & -0.40 ( 1)  & -0.14 ( 1)  &     --      & -0.07 ( 1)  &     --      & -0.21 ( 1)    & -0.33 ( 1)  & -0.34 ( 1)  & -0.23 ( 7)  &     --      &	   --     & -0.30 ( 7)  &     --      & -0.34 ( 1)   &     --     &      --      & -0.41 (22)  &     --      \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.04    &  $\pm$ 0.02 &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &     --      &  $\pm$ 0.10 &     --      &  $\pm$ 0.10   &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.04 &     --      &      --     &  $\pm$ 0.06 &     --      &  $\pm$ 0.10  &     --      &      --      &  $\pm$ 0.03 &     --	\\ 
26    & -0.56 (24)  & 19.00 ( 2)  &  0.31 (18)  & -0.45 (17)  & -0.41 ( 1)   & -0.59 ( 1)  & -0.21 ( 3)  & -0.24 ( 2)  & -0.27 ( 3)  & -0.31 ( 2)  & -0.31 ( 1)    & -0.33 ( 3)  & -0.40 ( 2)  & -0.21 ( 8)  & -0.32 ( 1)  & -0.27 ( 2)  & -0.36 (10)  & -0.35 ( 2)  & -0.38 ( 4)   & -0.39 ( 2)  & -0.39 ( 5)   & -0.42 (25)  & -0.42 (12)   \\  
   &  $\pm$ 0.02 &  $\pm$ 1.00 &  $\pm$ 0.04    &  $\pm$ 0.01 &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.01 &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.10   &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.05  &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.03 &  $\pm$ 0.04	\\ 
\rowcolor{lightgray} 																 
27    & -0.53 (23)  & 19.00 ( 2)  &  0.08 (27)  & -0.28 (19)  &     --       & -0.60 ( 1)  & -0.15 ( 1)  &     --      & -0.17 ( 1)  &     --      & -0.20 ( 1)    & -0.36 ( 2)  & -0.36 ( 2)  & -0.23 ( 9)  &     --      & -0.20 ( 1)  & -0.38 ( 9)  &     --      & -0.28 ( 2)   &     --      &      --      & -0.40 (22)  &     --      \\  
\rowcolor{lightgray} 																 
   &  $\pm$ 0.02 &  $\pm$ 1.50   &  $\pm$ 0.03  &  $\pm$ 0.01 &     --       &  $\pm$ 0.10 &  $\pm$ 0.10 &     --      &  $\pm$ 0.10 &     --      &  $\pm$ 0.10   &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03 &     --      &  $\pm$ 0.10 &  $\pm$ 0.02 &     --      &  $\pm$ 0.10  &     --      &      --      &  $\pm$ 0.03 &     --	\\ 
\hline\hline
\end{tabular}
\label{tab_elem1}
\end{table}
\end{landscape}



==> Perseus Complex (ArXiv)/tab3.tex <==
\begin{landscape}
\begin{table}[ht]
\centering
\caption{Iron, iron-peak and neutron-capture element abundances for the studied RSGs in the Perseus complex. Values are solar-scaled according to \citet{Grevesse98} solar reference. Numbers in parenthesis represent the number of lines used to determine chemical abundances}
\scriptsize
\addtolength{\tabcolsep}{-5.2pt}
\begin{tabular} {|c|cc|c|cc|cc|cc|cc|cc|c|c|cc|c|c|cc|c|cc|}
\hline 
\# & \multicolumn{2}{c|}{[FeI/H]} & [FeII/H] & \multicolumn{2}{c|}{[V/H]}& \multicolumn{2}{c|}{[Cr/H]} & \multicolumn{2}{c|}{[Mn/H]}&\multicolumn{2}{c|}{[Co/H]}& \multicolumn{2}{c|}{[Ni/H]}&[Cu/H] & [Zn/H]& \multicolumn{2}{c|}{[YI/H]} & [YII/H] & [Zr/H]&\multicolumn{2}{c|}{[Ce/H]}& [Nd/Fe] & \multicolumn{2}{c|}{[Dy/H]}\\
& NIR & OPT & OPT & NIR & OPT & NIR & OPT & NIR & OPT & NIR & OPT& NIR & OPT & NIR &NIR&NIR & OPT & OPT & OPT & NIR & OPT & OPT &  NIR & OPT \\
\hline
\rowcolor{lightgray} 							
1     & -0.35 (42)   & -0.32 ( 6)   & -0.35 ( 2)  & -0.26 ( 3)  &      --      & -0.27 (19)   & -0.30 ( 1)  & -0.25 ( 2)  &      --     & -0.23 ( 4)  &      --      & -0.28 ( 4)  &	   --     & -0.24 ( 1)   &      --     & -0.21 ( 1)  &      --      &      --      &	  --	  &	 --	         & -0.15 ( 1)  & -0.23 ( 2)  &      --      &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.03  &  $\pm$ 0.04  &  $\pm$ 0.10 &  $\pm$ 0.04 &      --      &  $\pm$ 0.04  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --     &  $\pm$ 0.06 &      --      &  $\pm$ 0.09 &      --      &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &      --      &      --      &	  --	  &	 --	         &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &	  --	   \\ 
2     & -0.35 (52)   & -0.32 (23)   & -0.35 ( 3)  & -0.36 ( 3)  & -0.26 (14)   & -0.36 (18)   & -0.30 ( 9)  & -0.37 ( 2)  & -0.38 ( 1)  & -0.44 ( 3)  & -0.33 ( 7)   & -0.39 ( 6)  & -0.36 ( 7)   & -0.21 ( 1)   &      --     & -0.21 ( 2)  &      --      &      --      & -0.30 ( 7)   & -0.11 ( 2)   & -0.15 ( 2)  & -0.23 ( 8)  & -0.26 ( 1)   & -0.22 ( 1)   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.01  &  $\pm$ 0.04  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.02  &  $\pm$ 0.12 &  $\pm$ 0.02  &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &      --      &      --      &  $\pm$ 0.03  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10  &  $\pm$ 0.10  \\ 
\rowcolor{lightgray} 																
3     & -0.27 (61)   & -0.25 (23)   & -0.23 ( 3)  & -0.39 ( 3)  & -0.26 (14)   & -0.37 (18)   & -0.30 ( 9)  & -0.42 ( 2)  & -0.32 ( 1)  & -0.36 ( 3)  & -0.25 ( 8)   & -0.25 ( 7)  & -0.23 ( 7)   & -0.25 ( 1)   &      --     & -0.31 ( 1)  &      --      &      --      & -0.39 ( 8)   & -0.12 ( 2)   & -0.15 ( 3)  & -0.23 ( 8)  & -0.19 ( 1)   & -0.20 ( 1)   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.02  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.08 &  $\pm$ 0.02  &  $\pm$ 0.11 &  $\pm$ 0.02  &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &      --      &      --      &  $\pm$ 0.05  &  $\pm$ 0.10  &  $\pm$ 0.03 &  $\pm$ 0.03 &  $\pm$ 0.10  &  $\pm$ 0.10  \\ 
4     & -0.38 (49)   & -0.35 (21)   & -0.28 ( 3)  & -0.40 ( 3)  & -0.39 (17)   & -0.37 (18)   & -0.35 ( 9)  & -0.26 ( 2)  & -0.38 ( 2)  & -0.42 ( 3)  & -0.34 ( 8)   & -0.28 ( 6)  & -0.39 ( 7)   & -0.24 ( 1)   &      --     & -0.36 ( 2)  & -0.30 ( 1)   & -0.30 ( 1)   & -0.36 ( 7)   & -0.10 ( 2)   & -0.10 ( 3)  & -0.18 ( 8)  & -0.27 ( 1)   & -0.27 ( 1)   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.01  &  $\pm$ 0.04  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.02  &  $\pm$ 0.11 &  $\pm$ 0.02  &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.02  &  $\pm$ 0.10  &  $\pm$ 0.03 &  $\pm$ 0.02 &  $\pm$ 0.10  &  $\pm$ 0.10  \\ 
\rowcolor{lightgray} 																
5     & -0.31 (48)   & -0.36 (21)   & -0.24 ( 3)  & -0.37 ( 3)  & -0.29 (17)   & -0.30 (16)   & -0.29 ( 7)  & -0.34 ( 1)  & -0.39 ( 1)  & -0.26 ( 4)  & -0.21 ( 6)   & -0.26 ( 5)  & -0.32 ( 8)   & -0.24 ( 1)   &      --     & -0.22 ( 2)  & -0.31 ( 1)   & -0.31 ( 1)   & -0.40 ( 7)   & -0.09 ( 2)   & -0.15 ( 3)  & -0.25 ( 6)  & -0.24 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.03 &  $\pm$ 0.01  &  $\pm$ 0.04  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.09 &  $\pm$ 0.02  &  $\pm$ 0.12 &  $\pm$ 0.02  &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.02  &  $\pm$ 0.10  &  $\pm$ 0.03 &  $\pm$ 0.03 &  $\pm$ 0.10  &	  --	   \\ 
6     & -0.33 (57)   & -0.29 (63)   & -0.34 ( 3)  & -0.33 ( 3)  & -0.36 (17)   & -0.29 (16)   & -0.33 ( 7)  & -0.42 ( 1)  & -0.38 ( 1)  & -0.39 ( 5)  & -0.39 ( 8)   & -0.31 ( 4)  & -0.35 ( 8)   & -0.34 ( 1)   & -0.30 ( 2)  & -0.17 ( 1)  &      --      &      --      & -0.23 ( 8)   & -0.05 ( 2)   & -0.15 ( 2)  & -0.06 ( 4)  & -0.25 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.17 &  $\pm$ 0.03 &  $\pm$ 0.02  &  $\pm$ 0.03  &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.09 &  $\pm$ 0.05  &  $\pm$ 0.12 &  $\pm$ 0.06  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &      --      &  $\pm$ 0.03  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																 
7     & -0.33 (57)   & -0.29 (63)   & -0.34 ( 3)  & -0.30 ( 2)  & -0.36 (16)   & -0.20 (18)   & -0.33 ( 7)  & -0.38 ( 1)  & -0.38 ( 1)  & -0.25 ( 6)  & -0.39 ( 7)   & -0.29 ( 6)  & -0.35 ( 7)   & -0.20 ( 1)   & -0.25 ( 2)  & -0.15 ( 2)  &      --      &      --      & -0.23 ( 8)   & -0.02 ( 1)   & -0.01 ( 3)  &  0.01 ( 5)  & -0.22 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.01  &  $\pm$ 0.02  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.06 &  $\pm$ 0.02  &  $\pm$ 0.05 &  $\pm$ 0.03  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &      --      &  $\pm$ 0.03  &  $\pm$ 0.10  &  $\pm$ 0.02 &  $\pm$ 0.02 &  $\pm$ 0.10  &	  --	   \\ 
8     & -0.30 (57)   & -0.30 (21)   & -0.29 ( 3)  & -0.35 ( 1)  & -0.42 (15)   & -0.36 (17)   & -0.39 ( 8)  & -0.19 ( 2)  &      --     & -0.39 ( 2)  & -0.37 ( 8)   & -0.23 ( 3)  & -0.39 ( 5)   &      --      &      --     & -0.31 ( 1)  & -0.30 ( 1)   & -0.30 ( 1)   & -0.31 (10)   & -0.32 ( 1)   & -0.21 ( 3)  & -0.22 (10)  & -0.19 ( 1)   & -0.16 ( 1)   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.04  &  $\pm$ 0.03 &  $\pm$ 0.10 &      --     &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.12 &  $\pm$ 0.03  &      --      &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.02  &  $\pm$ 0.10  &  $\pm$ 0.03 &  $\pm$ 0.03 &  $\pm$ 0.10  &  $\pm$ 0.10  \\ 
\rowcolor{lightgray} 																
9     & -0.29 (56)   & -0.33 (21)   & -0.26 ( 3)  & -0.42 ( 1)  & -0.40 (13)   & -0.37 (17)   & -0.35 ( 7)  & -0.19 ( 2)  &      --     & -0.37 ( 2)  & -0.38 ( 8)   & -0.27 ( 3)  & -0.34 ( 7)   &      --      &      --     & -0.26 ( 2)  & -0.37 ( 1)   & -0.37 ( 1)   & -0.28 (10)   & -0.20 ( 2)   & -0.20 ( 3)  & -0.27 (10)  & -0.23 ( 1)   &	  --	   \\
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.05  &  $\pm$ 0.03 &  $\pm$ 0.10 &      --     &  $\pm$ 0.10 &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.05  &      --      &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.04  &  $\pm$ 0.10  &  $\pm$ 0.03 &  $\pm$ 0.04 &  $\pm$ 0.10  &	  --	   \\ 
10    & -0.24 (60)   & -0.24 (22)   & -0.25 ( 3)  & -0.27 ( 1)  & -0.24 (16)   & -0.23 (18)   & -0.31 ( 7)  & -0.19 ( 2)  & -0.33 ( 2)  & -0.31 ( 2)  & -0.31 ( 8)   & -0.25 ( 2)  & -0.30 ( 7)   &      --      &      --     & -0.17 ( 1)  & -0.29 ( 1)   & -0.29 ( 1)   & -0.14 (10)   &  0.04 ( 1)   & -0.06 ( 2)  & -0.13 ( 9)  & -0.19 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.02  &  $\pm$ 0.04  &  $\pm$ 0.04 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.04  &  $\pm$ 0.10 &  $\pm$ 0.02  &      --      &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.04  &  $\pm$ 0.10  &  $\pm$ 0.09 &  $\pm$ 0.03 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
11    & -0.30 (61)   & -0.31 (20)   & -0.32 ( 2)  & -0.26 ( 1)  & -0.28 (16)   & -0.27 (18)   & -0.28 ( 8)  & -0.27 ( 3)  & -0.41 ( 2)  & -0.34 ( 2)  & -0.32 ( 8)   & -0.19 ( 3)  & -0.38 ( 2)   &      --      &      --     &      --     & -0.38 ( 1)   & -0.38 ( 1)   & -0.24 (10)   & -0.18 ( 1)   & -0.24 ( 3)  & -0.23 ( 9)  & -0.10 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.02  &  $\pm$ 0.05  &  $\pm$ 0.05 &  $\pm$ 0.16 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.02  &  $\pm$ 0.13 &  $\pm$ 0.10  &      --      &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.4  &  $\pm$ 0.10   &  $\pm$ 0.03 &  $\pm$ 0.07 &  $\pm$ 0.10  &	  --	   \\ 
12    & -0.26 (60)   & -0.25 (23)   & -0.29 ( 3)  & -0.25 ( 1)  & -0.28 (15)   & -0.28 (17)   & -0.31 ( 9)  & -0.11 ( 2)  &      --     & -0.31 ( 2)  & -0.27 ( 8)   & -0.32 ( 2)  & -0.34 ( 7)   &      --      &      --     &      --     & -0.22 ( 1)   & -0.22 ( 1)   & -0.17 (10)   &  0.08 ( 2)   &  0.01 ( 1)  & -0.14 (10)  & -0.10 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.01 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.05  &  $\pm$ 0.02 &  $\pm$ 0.10 &      --     &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.10 &  $\pm$ 0.5  &      --       &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.04  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
13    & -0.26 (56)   & -0.25 (23)   & -0.30 ( 3)  & -0.47 ( 1)  & -0.37 ( 9)   & -0.26 (17)   & -0.31 ( 8)  & -0.17 ( 3)  & -0.28 ( 1)  & -0.34 ( 2)  & -0.31 ( 7)   & -0.35 ( 3)  & -0.37 ( 8)   &      --      &      --     &      --     & -0.34 ( 1)   & -0.34 ( 1)   & -0.22 (10)   &  -0.37 ( 2)  & -0.07 ( 1)  & -0.17 ( 9)  & -0.20 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.14 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.09 &  $\pm$ 0.03  &      --      &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.03  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.02 &  $\pm$ 0.10  &	  --	   \\ 
14    & -0.31 (62)   & -0.32 (22)   & -0.33 ( 3)  & -0.25 ( 1)  & -0.28 (12)   & -0.33 (18)   & -0.34 ( 7)  & -0.25 ( 3)  & -0.40 ( 2)  & -0.39 ( 3)  & -0.35 ( 8)   & -0.30 ( 3)  & -0.39 ( 5)   &      --      &      --     & -0.25 ( 2)  & -0.45 ( 1)   & -0.45 ( 1)   & -0.35 (10)   & -0.16 ( 2)   & -0.13 ( 1)  & -0.29 (10)  & -0.17 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.04  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.09 &  $\pm$ 0.10 &  $\pm$ 0.07 &  $\pm$ 0.04  &  $\pm$ 0.14 &  $\pm$ 0.02  &      --      &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.01  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.04 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
15    & -0.28 (54)   & -0.27 (23)   & -0.30 ( 3)  &      --     & -0.27 (10)   & -0.22 (15)   & -0.30 ( 7)  & -0.24 ( 2)  & -0.27 ( 2)  & -0.43 ( 3)  & -0.28 ( 6)   & -0.36 ( 3)  & -0.35 ( 7)   &      --      &      --     &      --     & -0.17 ( 1)   & -0.17 ( 1)   & -0.08 (10)   &  0.17 ( 1)   &	--         & -0.02 ( 8)  & -0.02 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.02 &      --     &  $\pm$ 0.04  &  $\pm$ 0.04  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.11 &  $\pm$ 0.05  &  $\pm$ 0.09 &  $\pm$ 0.04  &      --      &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.06  &  $\pm$ 0.10  &	--         &  $\pm$ 0.03 &  $\pm$ 0.10  &	  --	   \\ 
16    & -0.26 (55)   & -0.23 ( 6)   & -0.26 ( 2)  & -0.35 ( 1)  &      --	   & -0.31 (18)   & -0.38 ( 1)  & -0.23 ( 2)  &      --     & -0.33 ( 3)  &      --      & -0.19 ( 3)  &  	   --     &      --      &      --     & -0.32 ( 2)  &      --      &      -       &	  --	  & -0.25 ( 2)   & -0.28 ( 1)  & -0.32 ( 2)  & -0.30 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &  $\pm$ 0.04  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --     &  $\pm$ 0.04 &      --      &  $\pm$ 0.02 &      --      &      --      &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &      --      &  	  --	  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
17    & -0.30 (61)   & -0.32 (19)   & -0.29 ( 3)  & -0.34 ( 1)  & -0.40 (13)   & -0.37 (18)   & -0.36 ( 7)  & -0.24 ( 1)  &      --     & -0.37 ( 3)  & -0.39 ( 7)   & -0.31 ( 3)  & -0.34 ( 6)   &   -0.19 ( 1) &      --     & -0.34 ( 2)  & -0.38 ( 1)   & -0.38 ( 1)   & -0.41 ( 8)   & -0.11 ( 2)   & -0.18 ( 2)  & -0.33 ( 8)  & -0.17 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.02  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.10 &      --     &  $\pm$ 0.10 &  $\pm$ 0.05  &  $\pm$ 0.08 &  $\pm$ 0.02  &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.03  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.05 &  $\pm$ 0.10  &	  --	   \\ 
18    & -0.29 (66)   & -0.26 (52)   & -0.22 ( 3)  & -0.27 ( 1)  & -0.30 (12)   & -0.33 (16)   & -0.33 ( 8)  & -0.16 ( 3)  & -0.08 ( 2)  & -0.48 ( 3)  & -0.34 ( 3)   & -0.29 ( 2)  & -0.34 ( 7)   &   -0.27 ( 1) &      --     &      --     & -0.14 ( 1)   & -0.14 ( 1)   & -0.19 ( 9)   &  0.08 ( 1)   &  0.01 ( 3)  & -0.02 ( 9)  & -0.25 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.04  &  $\pm$ 0.03  &  $\pm$ 0.03 &  $\pm$ 0.16 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.10 &  $\pm$ 0.02  &  $\pm$ 0.10  &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.04  &  $\pm$ 0.10  &  $\pm$ 0.07 &  $\pm$ 0.03 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
19    & -0.29 (55)   & -0.27 ( 9)   & -0.30 ( 2)  & -0.40 ( 1)  &      --	   & -0.39 (11)   & -0.42 ( 1)  & -0.15 ( 2)  &      --     & -0.35 ( 3)  &      --      & -0.36 ( 3)  &	   --     &  -0.23 ( 1)  &      --     & -0.31 ( 1)  &      --      &      --      &	  --	  &	 -0.23 ( 2)	 & -0.25 ( 1)  & -0.38 ( 2)  & -0.29 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &  $\pm$ 0.01  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --     &  $\pm$ 0.15 &      --      &  $\pm$ 0.06 &      --      &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &      --      &      --      &	  --	  &	 --	         &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10  &	  --	   \\ 
20    & -0.25 (59)   & -0.26 (20)   & -0.26 ( 3)  & -0.24 ( 1)  & -0.25 (12)   & -0.25 (17)   & -0.26 ( 7)  & -0.04 ( 2)  & -0.15 ( 1)  & -0.34 ( 2)  & -0.28 ( 8)   & -0.31 ( 2)  & -0.30 ( 7)   &      --      &      --     &      --     & -0.27 ( 1)   & -0.27 ( 1)   & -0.23 ( 4)   &  -0.18 ( 1)  &	--         & -0.16 ( 8)  & -0.15 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.04  &  $\pm$ 0.03 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.10 &  $\pm$ 0.02  &      --      &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.01  &  $\pm$ 0.10  &	--         &  $\pm$ 0.04 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
21    & -0.29 (61)   & -0.26 ( 6)   & -0.26 ( 2)  & -0.32 ( 1)  &      --	   & -0.37 (17)   & -0.38 ( 1)  & -0.05 ( 2)  &      --     & -0.37 ( 3)  &      --      & -0.23 ( 3)  &	   --     &  -0.16 ( 1)  &      --     &      --     &      --      &      --      &	  --	  &	 --	         & -0.19 ( 1)  & -0.22 ( 2)  & -0.28 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &  $\pm$ 0.04  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --     &  $\pm$ 0.03 &      --      &  $\pm$ 0.08 &      --      &  $\pm$ 0.10  &      --     &  --         &      --      &      --      &	  --	  &	 --	         &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10  &	  --	   \\ 
22    & -0.30 (53)   & -0.34 (18)   & -0.32 ( 2)  & -0.26 ( 1)  &  -0.37 ( 5)  & -0.29 (17)   & -0.36 ( 5)  & -0.31 ( 2)  & -0.33 ( 2)  & -0.38 ( 2)  & -0.35 ( 8)   & -0.18 ( 3)  & -0.29 ( 2)   &   -0.16 ( 1) &      --     &      --     & -0.32 ( 1)   & -0.32 ( 1)   & -0.25 ( 6)   &  -0.10 ( 1)  &	--         & -0.32 ( 6)  & -0.16 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.03  &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.03  &  $\pm$ 0.16 &  $\pm$ 0.06  &  $\pm$ 0.10  &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.03  &  $\pm$ 0.10  &	--         &  $\pm$ 0.03 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
23    & -0.30 (56)   & -0.28 ( 6)   & -0.24 ( 2)  & -0.32 ( 1)  &      --	   & -0.28 (17)   & -0.41 ( 1)  &      --     &      --     & -0.37 ( 3)  &      --      & -0.25 ( 3)  &	   --     &   -0.26 ( 1) &      --     &      --     &      --      &      --      &	  --	  &	 -0.02 ( 1)	 & -0.30 ( 1)  & -0.42 ( 2)  & -0.30 ( 1)   &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.03  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &  $\pm$ 0.04  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --     &  $\pm$ 0.06 &      --      &  $\pm$ 0.03 &      --      &  $\pm$ 0.10  &      --     &  --         &      --      &      --      &	  --	  & $\pm$ 0.10   &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10  &	  --	   \\ 
24    & -0.28 (54)   & -0.26 (54)   & -0.31 ( 3)  & -0.50 ( 1)  & -0.33 ( 5)   & -0.28 (16)   & -0.37 ( 7)  &  0.00 ( 2)  & -0.15 ( 2)  & -0.42 ( 3)  & -0.33 ( 5)   & -0.29 ( 2)  & -0.29 ( 7)   &   -0.23 ( 1) &      --     &      --     & -0.21 ( 1)   & -0.21 ( 1)   & -0.24 ( 8)   &	 0.08 (1)	 & -0.08 ( 3)  & -0.05 ( 8)  & -0.17 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.01  &  $\pm$ 0.05 &  $\pm$ 0.10 &  $\pm$ 0.05  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.10 &  $\pm$ 0.06  &  $\pm$ 0.10 &  $\pm$ 0.04  &  $\pm$ 0.10  &      --     &  --         &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.03  & $\pm$ 0.10   &  $\pm$ 0.04 &  $\pm$ 0.03 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
25    & -0.31 (46)   & -0.28 ( 6)   & -0.27 ( 1)  & -0.29 ( 1)  &      --	   & -0.29 (11)   & -0.37 ( 1)  & -0.15 ( 2)  &      --     & -0.25 ( 3)  &      --      & -0.27 ( 2)  &	   --     &  -0.24 ( 1)  &      --     & -0.16 ( 1)  &      --      &      --      &	  --	  &	 0.00 ( 1)	 & -0.22 ( 1)  & -0.31 ( 2)  &      --      &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.02  &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --     &  $\pm$ 0.03 &      --      &  $\pm$ 0.10 &      --      &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &      --      &      --      &	  --	  &	 $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &	  --	   \\ 
26    & -0.31 (54)   & -0.28 (16)   & -0.34 ( 3)  & -0.34 ( 1)  & -0.38 ( 8)   & -0.37 (14)   & -0.37 ( 7)  & -0.06 ( 2)  &      --     & -0.38 ( 3)  & -0.35 ( 7)   & -0.36 ( 3)  & -0.41 ( 6)   &   -0.13 ( 1) &      --     & -0.36 ( 2)  & -0.26 ( 1)   & -0.26 ( 1)   & -0.35 ( 8)   & -0.04 ( 2)   & -0.14 ( 3)  & -0.33 ( 8)  & -0.24 ( 1)   &	  --	   \\ 
      &  $\pm$ 0.02  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.10 &  $\pm$ 0.04  &  $\pm$ 0.04  &  $\pm$ 0.02 &  $\pm$ 0.10 &      --     &  $\pm$ 0.02 &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.04  &  $\pm$ 0.10  &    --       &  $\pm$ 0.10 &  $\pm$ 0.10  &  $\pm$ 0.10  &  $\pm$ 0.03  &  $\pm$ 0.10  &  $\pm$ 0.03 &  $\pm$ 0.03 &  $\pm$ 0.10  &	  --	   \\ 
\rowcolor{lightgray} 																
27    & -0.28 (36)   & -0.26 ( 6)   & -0.24 ( 2)  & -0.36 ( 1)  &      --	   & -0.34 (13)   & -0.38 ( 1)  & -0.18 ( 2)  &      --     & -0.33 ( 3)  &      --      & -0.30 ( 3)  &	   --     &   -0.23 ( 1) &      --     & -0.20 ( 2)  &      --      &      --      &	  --	  & -0.08 ( 1)   & -0.17 ( 1)  & -0.11 ( 2)  &      --      &	  --	   \\ 
\rowcolor{lightgray} 																
      &  $\pm$ 0.01  &  $\pm$ 0.03  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &  $\pm$ 0.02  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --     &  $\pm$ 0.03 &      --      &  $\pm$ 0.03 &      --      &  $\pm$ 0.10  &      --     &  $\pm$ 0.10 &      --      &      --      &	  --	  &  $\pm$ 0.10  &  $\pm$ 0.10 &  $\pm$ 0.10 &      --      &	  --	   \\ 
\hline\hline
\end{tabular}
\label{tab_elem2}
\end{table}
\end{landscape}

